Finite element method. Detailed proofs to be formalized in Coq

To obtain the highest confidence on the correction of numerical simulation programs for the resolution of Partial Differential Equations (PDEs), one has to formalize the mathematical notions and results that allow to establish the soundness of the approach. The finite element method is one of the popular tools for the numerical resolution of a wide range of PDEs. The purpose of this document is to provide the formal proof community with very detailed pen-and-paper proofs for the construction of the Lagrange finite elements of any degree on simplices in positive dimension.

==> algo_fem.tex <==
%%======
\subsection{Mesh}
Let $\Omega \subset \matR^3$ be an open bounded connected polyhedral domain.
We recall that $\overline{A}$ is the closure of a set $A \subset{\matR^{d}}$ ($d=1,2,3$).
The mesh of $\Omega$ is made up of:
\begin{itemize}
\item a set of $N_V>0$ vertices $\calV= \{\vv_i \in \matR^3 \st i=1,\ldots,N_V\}$.
It is generally stored as a vector of triplets, 
\[
(\vv_i)_{i=1,\ldots,N_V}  = (x_i, y_i, z_i)_{i=1,\ldots,N_V} \in \matR^{(3\times N_V)}.
\]
The vertex $\vv_i$ is generally defined by its cartesian coordinates.
\item a set of $N_K>0$ geometric elements 
\[
\calT_h = \{ K_j  \subset \ovOmega \st  j=1,\ldots,N_K\},
\]
and $h \in \matR \ (h>0)$ is defined by 
\[
h = \max_{j=1,\ldots,N_K} \diam(K_j).
\] 
A geometric element 
$K_j = \dps [\vv_{v^1_j}, \vv_{v^2_j}, \ldots, \vv_{v^{n^K_V}_j}] \subset \ovOmega$ 
is the convex hull of its vertices (when these vertices are properly numbered).
$K_j$ is entirely defined by $\tilde{K}_j$, the list of the indices of its
$n^K_V$ vertices. 
Thus, $\calT_h$ is often stored as a list of tuple 
\[
(\tilde{K}_j)_{j=1,\ldots,N_K} 
= (v^1_j, v^2_j, \ldots, v^{n^K_V}_j)_{j=1,\ldots,N_K} \in \matN^{(n^K_V\times N_K)},
\] 
where $n^K_V$ is the number of vertices per geometric element. In a geometric
element, all indices are different: $\forall j = 1,\ldots, N_K, 
\forall i_1, i_2=1,\ldots, n^K_V, \ i_1 \neq i_2 \implies v^{i_1}_j \neq v^{i_2}_j$  .
The list $\tilde{K}_j$ is ordered so that the element $K_j$ has a strictly 
positive (Lebesgue) measure and is not self intersecting. 
\\
(For a tetrahedric mesh, $n^K_V = 4$, as there are $4$ vertices per tetrahedron.)

\item (often) a set of $N_F>0$ geometric boundary elements 
\[
\calF_h = \{ F_k  \subset \ovOmega \st  k=1,\ldots,N_F\},
\]
that define the skin of the mesh, \ie{} the closed mesh made up of faces that live
on the boundary $\pOmega$ of the domain. It is closed in the sense that there
is no hole in the boundary mesh: $\pOmega = \bigcup_{k=1}^{N_F} F_k$.\\
A geometric boundary element 
$F_k = \dps [\vv_{v^1_k}, \vv_{v^2_k}, \ldots, \vv_{v^{n^F_V}_k}] \subset \pOmega$ 
is entirely defined by $\tilde{F}_k$, the list of the indices of its $n^F_V$ vertices.
Thus $\calF_h$ is often stored as a tuple 
\[
(\tilde{F}_k)_{k=1,\ldots,N_F} = (v^1_k, v^2_k, \ldots, v^{n^F_V}_k)_{k=1,\ldots,N_F} 
\in \matN^{(n^F_V\times N_F)},
\]
where $n^F_V$ is the number of vertices per faces. 
The list $\tilde{F}_k$ is ordered so that the element $F_k$ has a positive 
measure (in dimension 2), 
is not self intersecting and is oriented towards the exterior of $\Omega$. 
\\
(For a tetrahedric mesh, $n^F_V = 3$, as the faces of a tetrahedron are triangles.)
\end{itemize}

%\begin{remark}
In this presentation, for the sake of simplicity, we assume that 
the mesh is made up of only {\em one} type of geometric element,
so that $n^K_V$ is constant per element. We also assume that
the element is such that $n^F_V$ is constant ($n^F_V$ could be varying 
for a single element: think of a prism element, whose faces are 
2 triangles and 3 quadrangles). 
In the code \felisce, there is no such assumption: a mesh can 
have tetrahedra and hexahedra... 
%\end{remark}

A mesh is well-defined (it is said to be conforming),
if the following additional properties are satisfied:
\[
\dps \overline{\Omega} = \bigcup_{j=1}^{N_K} K_j,
\qquad
\dps 
i\neq j \implies K_i \cap K_j = 
\left\{\begin{array}{l}
\emptyset, \\
\mbox{a vertex } \vv_p \in \calV, \\
\mbox{an edge } [\vv_{p_1}, \vv_{p_2}] , \ \vv_{p_k} \in \calV, \ \forall k=1,2, \\
\mbox{a face } [\vv_{p_1}, \ldots, \vv_{p_{n^F_V}}] , \ \vv_{p_k} \in \calV, 
\ \forall k=1,\ldots, n^F_V. \\
\end{array}\right. 
\]

Note that when $K_i \cap K_j$ is a face, it cannot be 
in $\calF$, as a face of the skin touches only one element.

Often, the geometric elements, the boundary geometric elements and 
the vertices have labels that allow the user to define
properties or boundary conditions to specific zones of the domain.

%\begin{remark}
In this presentation, for the sake of simplicity, we will omit all the details
concerning the boundary conditions, and consequently on the skin mesh.
%\end{remark}

%%======
\subsection{Reference geometric element}
Define a reference geometric element  in dimension $d$ ($d=1,2,3$),
$\hK = [\hvv_1,\ldots, \hvv_{n^K_V}] \subset \matR^d$ as 
a compact, connected, polytope with non empty interior. It can be typically 
the unit rectangular simplex 
\begin{equation} 
\label{e:ref:simplex}
\hK = [\hvv_0, \ldots, \hvv_d] =  
\left\{\hxx \in \matR^d \st 0\leq \hx_i \leq 1, i=1,\ldots,d,\ \mbox{ and }
\sum_{i=1}^d\hx_i \leq 1\right\},
\end{equation}
and we choose by convention here that 
$\hvv_0 = 0$ and $\hvv_i$ is such that $\hx_i =1$ and 
$\hx_{j} =0$ ($j\neq i$). 

Other typical examples are the centered and unit hypercubes 
\begin{equation} 
\label{e:ref:hexhedron}
\hC_c =  [\hvv_1, \ldots , \hvv_{2^d}]= [-1,1]^d, \qquad
\hC_u =  [\hvv_1, \ldots , \hvv_{2^d}]= [0,1]^d.
\end{equation}
For the numbering of the vertices in these hypercubes, see~\cite{eg:fe1:21}.

%%======
\subsection{Geometric mapping}
Whenever possible, the computations over a geometric element 
$K \subset \ovOmega$ are performed on the chosen reference 
geometric element $\hK$. It is necessary to relate $K$ and $\hK$.

\begin{figure}[htb]
  \centering
\begin{tikzpicture}
\draw[step=.5cm, very thin, black!20] (-4,-4) grid (8,2.2) ;
\coordinate[label=left : $\hvv_0$] (a) at (-3,-3) ;
\coordinate[label=above : $\hvv_2$] (c) at (-3,0) ;
\coordinate[label=right : $\hvv_1$] (b) at (0,-3) ;

\coordinate[label=left : $0$] (0) at (-2.7,-3.3) ;
\coordinate[label=above : $1$] (2) at (-3.3,-0.3) ;
\coordinate[label=right : $1$] (1) at (-0.3,-3.3) ;

\draw[thick] (a)--(b)--(c)--cycle ;

\coordinate[label=left : \textcolor{black}{$\vv_0 = \phigeo^{K} (\hvv_0)$}] (A) at (3,-1) ;
\coordinate[label=above : \textcolor{black}{$\vv_2 = \phigeo^{K} (\hvv_2) $}] (C) at (7,1) ;
\coordinate[label=right : \textcolor{black}{$\vv_1 = \phigeo^{K} (\hvv_1) $}] (B) at (5.5,-3) ;
\draw[thick] (A)--(B)--(C)--cycle ;

\node (arrow) [] {};
    \draw[-latex,blue, very thick] ($(arrow.north west)+(-1,-1)$) arc
    [start angle=160,
     end angle=70,
     x radius=3.8cm,
     y radius =2cm] ;
     
\coordinate[label=above : \textcolor{blue}{$\phigeo^{K}$}] (T) at (1,0.5) ;
% K^hat
\coordinate[label=left : \textcolor{blue}{$\hK$}] (Khat) at (-1.7,-2) ;
% K 
\coordinate[label=right : \textcolor{blue}{$K$}] (Khat) at (5,-1) ;

% The expressions of Tk
\coordinate[label=above : \textcolor{black}{$\phigeo^{K} : \hK \ni \hxx \mapsto \sum_{i=1}^{n^K_V} \hcalL_i (\hxx) \ \vv_i$} \ affine] (T) at (-1.1,1.5) ;

\coordinate[label=above : \textcolor{black}{$\phigeo^{K}(\hK)=K \ \wedge \ (\phigeo^{K})^{-1}(K)=\hK$}] (T) at (-1.7,0.9) ;
\end{tikzpicture}
  \caption{%
    Example of a geometric mapping. In this simplicial case, the
    transformation is affine, mapping a reference right unit triangle
    to a current triangle.}
  \label{fig:FEM-map-bis}
\end{figure}

For each geometric element $K$, define the geometric mapping 
\begin{equation} 
  \label{e:phi-geo}
  \phigeo : 
  \left\{\begin{array}{rcll}
  \hK &\rightarrow& K \\
  \hxx &\mapsto&  \xx = \phigeo(\hxx)
  \end{array}\right. ,
\end{equation}
and  $\phigeo$ is a $\calC^1$ diffeomorphism. 
It is generally a polynomial of $\calP(\matR^3,\matR^3)$. 

Then define the jacobian matrix of $\phigeo$ by 
\begin{equation} 
  \label{e:jac:phi:geo}
  \jacphigeo : 
  \left\{\begin{array}{rcll}
  \hK &\rightarrow& \calM_{3,3}(\matR) \\
  \hxx &\mapsto & \jacphigeo(\hxx) = \Diff \phigeo(\hxx)
  \end{array}\right. .
\end{equation}

%%======
\subsection{Interpolation}
In the elements, one needs to define the finite functional space where one looks for
the solution.  Here is a simple example, among many others.
%%======
\subsubsection{Lagrange polynomial}

Let $K\subset \ovOmega$ be a geometric nondegenerate element, 
$K = \dps [\vv_{v^1}, \vv_{v^2}, \ldots, \vv_{v^{n^K_V}}]$.

Then we can define the Lagrange polynomials of $\calP(\matR^3)$ 
(it is a linear independent family, and  
a basis of the vector space of polynomials $\matP$ or $\matQ$ to be defined...)
\[
\calL^K_i(\vv_{v^j}) = \delta_{ij}, \quad i,j=1,\ldots, n^K_V.
\]
such that for all polynomials $p$ in $\matP$, 
\[
p = \sum_{i=1}^{n^K_V} p(\vv_{v^i}) \calL^K_i.
\]

%%======
\subsection{Quadrature rules}
A quadrature rule on an element $K$ is
a function that approximates the integral of functions over $K$. 
\begin{equation}
  \label{e:def:quad:rule}
  I^K_\calQ(f) = \sum_{i_q=1}^{N_q} f(\xxi_{i_q}) \omega_{i_q} \in \matR, \qquad
\forall f \in \calC^0(K, \matR).
\end{equation}

Thus the data of a quadrature rule is defined by 
\begin{equation}
  \label{e:quad-rule-data}
  \calQ  = (N_q,   (\xxi_{i_q})_{i_q=1,\ldots,N_q}, 
  (\omega_{i_q})_{i_q=1,\ldots,N_q}, \degq ),
\end{equation}
where $N_q \in \matN \ (N_q>0)$ is the number of points of the
quadrature rule, $\xxi_{i_q} \in K$ are the quadrature points (where the
function needs to be computed),  $\omega_{i_q} \in \matR$
are the weights of the quadrature rule, $\degq$ is the degree
of exactness  (or quadrature order) of the approximation, defined by:

\begin{equation}
  \label{e:quad-rule-deg-exact}
  \degq  = \max_{k\in\matN} \left\{   I^K_\calQ(p) = \int_K p(\xx) d\xx \st 
  \forall p \in \matPkd \right\}.
\end{equation}
Note that $\degq$ is entirely defined from the $\xxi_{i_q}$ and the $\omega_{i_q}$.
One has usually estimates of the type
\begin{equation}
  \label{e:quad:rule:deg:estimate}
  \exists \alpha > 0, \forall f, \exists C(f) > 0 \quad 
  \left| I^K_\calQ(f) - \int_K f(\xx) d\xx \right| \leq C(f) \; (\diam(K))^\alpha, 
\end{equation}
for regular enough functions $f$.
For instance, using Taylor expension, one has~\cite{eg:tpf:04}
\begin{equation}
  \label{e:quad-rule-deg-estimate-Taylor}
  \exists c > 0, \forall f \in \calC^{\degq+1}(K) \quad 
  \left| I^K_\calQ(f) - \int_K f(\xx) d\xx \right| \leq c  \; h^{\degq+1}_K 
  \sup_{\xx \in K, |\alpha| = \degq+1} |\p^\alpha f(\xx)| \; \meas(K). 
\end{equation}

%%======
\subsection{Model problem: Poisson}
We want to solve the Poisson problem
\begin{equation} \label{eq:lapl:strong}
  \begin{array}{rcll}
    \dps \mbox{Find } p  \mbox{ such that} & & &\\
    \dps - \Delta p & = & g & \mbox{in } \Omega\\
    p & = & 0 & \mbox{on } \Gamma = \partial \Omega,
  \end{array}
\end{equation}
which can be reformulated in a weak form
\begin{equation}\label{eq:lapl:weak}
  \begin{array}{rcll}
    \dps \mbox{Find } p \in H^{1}_{0}(\Omega) \mbox{ such that} & & &\\
    \dps \int_{\Omega} \nabla p \cdot \nabla q  & = & \dps \int_{\Omega} g\, q, &
    \dps \forall q \in H^{1}_{0}(\Omega).
  \end{array}
\end{equation}
To this end, we define a finite element space $V_h \subset H^{1}_{0}(\Omega)$,
supported by the mesh $\calT_h$. The Finite Element Method (FEM) consists in solving
\begin{equation}\label{eq:lapl:weak:discr}
  \begin{array}{rcll}
    \dps \mbox{Find } p_h \in V_h \mbox{ such that} & & &\\
    \dps \int_{\Omega} \nabla p_h \cdot \nabla q_h  & = & \dps \int_{\Omega} g\, q_h, &
    \dps \forall q_h \in V_h.
  \end{array}
\end{equation}

Define a basis $\{\phi_j: j=1,\ldots,N_n\}$  of $V_h$, where 
$N_n$ is the total number of ``degrees of freedom'' (\ie{} the dimension) of~$V_h$. 
Write $p_h=\dps \sum_{j=1}^{Nn}P^h_j\phi_j$
and take successively $q_h = \phi_i$, in~\eqref{eq:lapl:weak:discr}
to obtain
\begin{equation}\label{eq:lapl:weak:discr:linsys}
  \begin{array}{rcll}
    \dps \mbox{Find } P^h \in \matR^{N_n} \mbox{ such that}\\
    \dps \sum_{j=1}^{N_n} \left(
      \int_{\Omega} \nabla \phi_j \cdot \nabla \phi_i
    \right) P^h_j & = & \dps \int_{\Omega} g\,\phi_i, &
    \dps \forall i=1,\ldots,N_n,
  \end{array}
\end{equation}
which is the line $i$ of the linear system 
\begin{equation}\label{eq:lapl:weak:discr:linsys:Axb}
AP^h = b, \qquad \mbox{ where }
\left\{\begin{array}{rcll}
\dps A_{ij} &=&  \dps \int_{\Omega} \nabla \phi_j \cdot \nabla \phi_i, & i,j =1,\ldots, N_n\\
\dps b_{i}  &=&  \dps\int_{\Omega} g\,\phi_i, & i =1,\ldots, N_n. 
\end{array}\right.
\end{equation}

In problem~\eqref{eq:lapl:weak:discr:linsys}, the integrals are generally computed
as follows: decompose over all the elements of the mesh, use a geometric
transformation to integrate over a reference element (typically a unit right
tetrahedron), and use a quadrature formula on this reference element:
\begin{equation}\label{eq:int:transf:quad}
  \begin{array}{rcll}
    \dps \int_{\Omega} \nabla \phi_j \cdot\nabla \phi_i & = &
    \dps \sum_{K \in \calT_h} \int_{K} \nabla \phi_j \cdot \nabla \phi_i &
    \hspace*{-2.3cm} (K \mbox{ is the current element})\\
    & = &
    \dps \sum_{j=1}^{N_K} \int_{\hat{K}} (\jacphigeo)^{-T} \hat{\nabla} \hat{\phi}_j
    \cdot (\jacphigeo)^{-T} \hat{\nabla} \hat{\phi}_i \; |\det \jacphigeo| &
    \hspace*{-2.3cm} (\hat{K} \mbox{ is the reference elt})\\
    & \approx &
    \dps \sum_{j=1}^{N_K} \sum_{i_g = 1}^{N_q}  \left(
      (\jacphigeo)^{-T} \hat{\nabla} \hat{\phi}_j \cdot
      (\jacphigeo)^{-T} \hat{\nabla} \hat{\phi}_i \; |\det (\jacphigeo)|
    \right)(\hxxi_{i_g}) \; \hatom_{i_g}, &
  \end{array}
\end{equation}
where~$J_K$ is the Jacobian matrix of the geometric transformation that maps
the reference element~$\hat{K}$ to the current element~$K$, and~$\hxx_{i_g}$,
and~$\hatom_{i_g}$ are the Gauss points and weights of the quadrature formula
over~$\hK$.

%%======
\subsection{FEM algorithm}

Here is a possible algorithm for the FEM.

\begin{enumerate}
  \item Read the mesh.
  \item Build static data:
    \begin{enumerate}
      \item Define the reference element 
        $\hK = [\hvv_1,\ldots, \hvv_{n^K_V}]  \subset \matR^3$. 
      \item Choose the quadrature rule on $\hK$
\[
\calQ  = (N_q, 
  (\hxx_{i_q})_{i_q=1,\ldots,N_q}, 
  (\hatom_{i_q})_{i_q=1,\ldots,N_q} ),
\]
        with $N_q \in \matN \ (N_q>0)$, 
        $\hxx_{i_q} \in  \hK$, 
        and  $\hatom_{i_q} \in \matR$.
      \item Choose the geometric mapping that maps the 
        geometric reference element $\hK$
        onto a ``current'' geometric element $K \subset \ovOmega$,
\[
\phigeo : \hK \rightarrow K, \quad \xx = \phigeo(\hxx),
\]
and  $\phigeo$ is bijective, and generally a polynomial of $\calP(\matR^3)$. 
      \item Choose the approximation in the reference element $\hK$
\[
\hphi : \hK \rightarrow \matR, \quad \hphi(\hxx) \in \matR,
\]
and  $\hphi$ is a polynomial of $\calP(\matR^3)$. 
    \item Compute and store 
    \end{enumerate}
\end{enumerate}

